Mu2e-II: Muon to electron conversion with PIP-II

An observation of Charged Lepton Flavor Violation (CLFV) would be unambiguous evidence for physics beyond the Standard Model. The Mu2e and COMET experiments, under construction, are designed to push the sensitivity to CLFV in the mu to e conversion process to unprecedented levels. Whether conversion is observed or not, there is a strong case to be made for further improving sensitivity, or for examining the process on additional target materials. Mu2e-II is a proposed upgrade to Mu2e, with at least an additional order of magnitude in sensitivity to the conversion rate over Mu2e. The approach and challenges for this proposal are summarized. Mu2e-II may be regarded as the next logical step in a continued high-intensity muon program at FNAL.

==> GNUmakefile <==
#------------------------------------------------------------------------------
# primary source: .eps
# store ROOT plots in .eps format, make .png and .pdf out of .eps files
#------------------------------------------------------------------------------
dir=.

note := main

tex_files := $(note).tex # $(wildcard *.tex)

pdfs := $(patsubst figures/eps/%.eps, figures/pdf/%.pdf,  $(wildcard figures/eps/*.eps ))

pngs := $(patsubst figures/eps/%.eps, figures/png/%.png, $(wildcard figures/eps/*.eps ))

figures/pdf/%.pdf: figures/eps/%.eps
	ps2pdf -dEPSCrop $? $@

figures/png/%.png: figures/eps/%.eps
	convert -density 400 -depth 8 -quality 85  $? $@

pdf: $(pdfs) 
# 	echo $?
png: $(pngs) 
# 	echo $?

local_bstinputs := ${BSTINPUTS}:${PWD}:
local_bibinputs := ${BIBINPUTS}:${PWD}:
local_texinputs := ${TEXINPUTS}:${PWD}:

note: $(tex_files) pdf
	if [ ! -d tmp ] ; then mkdir tmp ; fi ; \
	export BSTINPUTS=$(local_bstinputs) ; export BIBINPUTS=$(local_bibinputs) export TEXINPUTS=$(local_texinputs) ; \
	pdflatex -interaction=batchmode -output-directory=tmp $^  ; \
	cd tmp; bibtex $(note).aux; cd ..; \
	pdflatex -interaction=batchmode -output-directory=tmp $^  ; \
	pdflatex -output-directory=tmp $^  ; \
	cp tmp/$(note).pdf .

quiet: $(tex_files) pdf
	if [ ! -d tmp ] ; then mkdir tmp ; fi ; \
	export BSTINPUTS=$(local_bstinputs) ; export BIBINPUTS=$(local_bibinputs) export TEXINPUTS=$(local_texinputs) ; \
	pdflatex -interaction=batchmode -output-directory=tmp $^  ; \
	cd tmp; bibtex $(note).aux; cd ..; \
	pdflatex -interaction=batchmode -output-directory=tmp $^  ; \
	pdflatex -interaction=batchmode -output-directory=tmp $^  ; \
	cp tmp/$(note).pdf .


all: pdf note
	echo $(pdfs)
	echo $?

